The Oscars of AI Theater: A Survey on Role-Playing with Language Models

This survey explores the burgeoning field of role-playing with language models, focusing on their development from early persona-based models to advanced character-driven simulations facilitated by Large Language Models (LLMs). Initially confined to simple persona consistency due to limited model capabilities, role-playing tasks have now expanded to embrace complex character portrayals involving character consistency, behavioral alignment, and overall attractiveness. We provide a comprehensive taxonomy of the critical components in designing these systems, including data, models and alignment, agent architecture and evaluation. This survey not only outlines the current methodologies and challenges, such as managing dynamic personal profiles and achieving high-level persona consistency but also suggests avenues for future research in improving the depth and realism of role-playing applications. The goal is to guide future research by offering a structured overview of current methodologies and identifying potential areas for improvement. Related resources and papers are available at https://github.com/nuochenpku/Awesome-Role-Play-Papers.

==> figures/test_flow.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
]
\tikzstyle{cause_leaf}=[my-box, minimum height=1.5em,
    fill=harvestgold!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\tikzstyle{detect_leaf}=[my-box, minimum height=1.5em,
    fill=cyan!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\tikzstyle{mitigate_leaf}=[my-box, minimum height=1.5em,
    fill=lightgreen!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\tikzstyle{eval_leaf}=[my-box, minimum height=1.5em,
    fill=pink!10, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\tikzstyle{sys_leaf}=[my-box, minimum height=1.5em,
    fill=orange!10, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\begin{figure*}[]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=4.0em,font=\scriptsize,}{},
            where level=2{text width=7.5em,font=\scriptsize,}{},
            where level=3{text width=7.2em,font=\scriptsize,}{},
            where level=4{text width=6.4em,font=\scriptsize,}{},
            [
                Role-Playing Langauge  Agents, ver, color=carminepink!100, fill=carminepink!15,
                text=black
                [
                    Foundation \\ Models and \\ Architectures (\S \ref{sec:causes}), color=harvestgold!100, fill=harvestgold!100, text=black
                    [
                        None-pretrained, color=harvestgold!100, fill=harvestgold!60,  text=black
                        [
                        {\eg~Per-S2SA \cite{zhang-etal-2018-personalizing}, DeepCopy \cite{yavuz-etal-2019-deepcopy}, Per-CVAE \cite{song2019exploiting}, GDR \cite{song-etal-2020-generate}}
                            , cause_leaf, text width=36em
                        ]
                        ]
                    [
                        PLM-based, color=harvestgold!100, fill=harvestgold!60, text=black
                        [
                        {\eg~ConvAI2 \cite{dinan2019second}, LIC \cite{golovanov-etal-2019-large}, BOB \cite{song-etal-2021-bob}, Attention Routing \cite{Zheng_Zhang_Huang_Mao_2020}}
                        % \citet{jang2022call}}
                        ,  cause_leaf, text width=36em
                        ]
                    ]
                    [
                        LLM-based, color=harvestgold!100, fill=harvestgold!60, text=black
                        [
                                {\eg~CharacterGLM \cite{zhou2023characterglm}, Character-LLM \cite{shao2023character}, RoleLLM \cite{wang2023rolellm}, ChatHaruhi \cite{li2023chatharuhi},\\ ChatPlug \cite{tian2023chatplug}, DITTO \cite{lu2024large}}
                                , cause_leaf, text width=36em
                            % ]
                            % ]
                        ]

                    ] 
                ]
                [
                    Data(\S \ref{sec:detection_and_benchmark}), color=cyan!100, fill=cyan!100, text=black
                    [
                        Persona-based RPDAs, color=cyan!100, fill=cyan!60, text=black
                        [
                            Employing Crowdsourced \\ Workers, color=cyan!100, fill=cyan!30, text=black
                            [
                                {\eg~Persona-Chat \cite{zhang-etal-2018-personalizing}, Focus \cite{DBLP:journals/corr/abs-2112-08619}, KvPI \cite{song2020profile},\\ WOW \cite{dinan2018wizard}, ConvAI2 \cite{dinan2019second}}
                                , detect_leaf, text width=27em
                            ]
                        ]
                        [
                            Extracting from    Social \\Media, color=cyan!100, fill=cyan!30, text=black
                            [
                                {\eg~Pchatbot \cite{DBLP:conf/sigir/QianLZGMZLDW21}, PeDialog \cite{DBLP:journals/corr/abs-1901-09672}, LiveChat \cite{gao2023livechat},\\ P-Ubuntu \cite{li2021dialogue}, Friends-QA \cite{DBLP:conf/sigdial/YangC19}}
                                , detect_leaf, text width=27em
                            ]
                        ]
                    ]
                    [
                        Character-based RPDAs, color=cyan!100, fill=cyan!60, text=black
                        [
                            LLMs as  Data Generator, color=cyan!100, fill=cyan!30, text=black
                            [
                                {\eg~InCharacter \cite{wang2024incharacter}, RoleInteract \cite{chen2024roleinteract}, Rolebench \cite{wang2023rolellm}, \\CharacterDia \cite{zhou2023characterglm}, MBTI-S2Conv \cite{tu2023characterchat}
                                }
                                , detect_leaf, text width=27em
                            ]
                        ]
                        [
                            Extracting from \\ Literary Resources, color=cyan!100, fill=cyan!30, text=black
                            [
                                {\eg~HPD \cite{chen2023large}, CharacterEval \cite{tu2024charactereval}, RoleEval \cite{wang2023rolellm}, \\CharacterDia \cite{zhou2023characterglm} }
                                , detect_leaf, text width=27em
                            ]
                        ]

                        [
                            Extracting from Online\\ Role-Playing Platforms, color=cyan!100, fill=cyan!30, text=black
                            [
                                {\eg~Dolphin \cite{chen2024compress}, RoleEval \cite{shen2024roleeval}, PIPPO \cite{gosling2023pippa}}
                                , detect_leaf, text width=27em
                            ]
                        ]

                        [
                            Human Role-Playing, color=cyan!100, fill=cyan!30, text=black
                            [
                                {\eg~CharacterDia \cite{zhou2023characterglm}, \citet{zhang2024unveiling}}
                                , detect_leaf, text width=27em
                            ]
                        ]



                        
                    ]
                ]
                [
                    Modeling  \\ Alignment (\S \ref{sec:mitigating}), color=lightgreen!100, fill=lightgreen!100, text=black
                    [
                        Parameter-Tuning, color=lightgreen!100, fill=lightgreen!60, text=black
                        [
                            Post-Training  (Pre-training) , color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                             {\eg~ChatPlug \cite{tian2023chatplug}, \citet{DBLP:conf/emnlp/HuangD0M22}
                                    }, mitigate_leaf, text width=27em
                            ]
                            
                        ]
                        [
                            Supervised Fine-tuning , color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                            {\eg~RoCIT \cite{wang2023rolellm},
                            BOB \cite{song-etal-2021-bob}, RoleLLM \cite{wang2023rolellm}\\
                            CharacterGLM\cite{zhou2023characterglm}, Character-LLM \cite{shao2023character}, PLATO-LTM \cite{DBLP:conf/acl/XuGWNW0W22}}, mitigate_leaf, text width=27em
                            ]
                        ]
                        [
                            Self-Alignment, color=lightgreen!100, fill=lightgreen!40, text=black
                           [
                           {\eg~CharacterGLM \cite{wang2023rolellm},
                           \citet{lu2024large}}, mitigate_leaf, text width=27em
                           ]
                        ]
                        [
                            Parameter-Efficiency \\ Tuning, color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                            {\eg~PersonaPKT \cite{DBLP:conf/sustainlp/HanGJYZLG23},
                            Neeko \cite{yu2024neeko}}, mitigate_leaf, text width=27em
                            ]
                        ]
                        [
                             Reinforcement Learning , color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                            {\eg~COMEDY \cite{chen2024compress}, \citet{shea-yu-2023-building}}, mitigate_leaf, text width=27em
                            ]

                        ]
                        
                    ]
                    [
                        Parameter-Frozen, color=lightgreen!100, fill=lightgreen!60, text=black
                        [
                            In-context Learning \\Prompting, color=lightgreen!100, fill=lightgreen!40, text=black
                        [
                        {\eg~\citet{chen2023large}, \citet{shea-yu-2023-building}, \citet{shen2024roleeval}}, mitigate_leaf, text width=27em
                        ]
                        ]
                        [
                           Retrieval-based Augmented\\Generation, color=lightgreen!100, fill=lightgreen!40, text=black
                    [{\eg~RECAP\cite{liu-etal-2023-recap}, Narrativeplay\cite{shea-yu-2023-building}, LAMP \cite{salemi2024lamp} }, mitigate_leaf, text width=27em]
                    ]
                    ]

       
                    ]

            [
            System \\ Architecture (\S \ref{sec:mitigating}), color=orange!100, fill=orange!100, text=black
            [
           Memory, color=orange!100, fill=orange!60, text=black
            [
            Memory Sources, color=orange!100, fill=orange!40, text=black[
            User-Agent Interaction, color=orange!100, fill=orange!30, text=black[
              {\eg~\citet{DBLP:conf/acl/XuGWNW0W22}, \citet{JiangPersonaLLMIT}, RoleInteract \cite{chen2024roleinteract}}, sys_leaf, text width=19em
              ]
              ]
               [Agent-Agent Interaction, color=orange!100, fill=orange!30, text=black[
              {\eg~\citet{maas2023infinity}, Generative Agent \cite{park2023generative}}, sys_leaf, text width=19em
              ]
              ]         
            ]
            [
            Memory Usage, color=orange!100, fill=orange!40, text=black[
            Retrieval-based, color=orange!100, fill=orange!30, text=black[
              {\eg~PLATO-LTM \cite{DBLP:conf/acl/XuGWNW0W22}, \citet{bae-etal-2022-keep} }, sys_leaf, text width=19em
              ]
              ]
               [Compressive-based, color=orange!100, fill=orange!30, text=black[
              {\eg~COMEDY \cite{chen2024compress}, \citet{wang2023recursively}}, sys_leaf, text width=19em
              ]
              ]         
            ]
            ]
            [
             Planning, color=orange!100, fill=orange!60, text=black[
              Planning Formulation, color=orange!100, fill=orange!40, text=black
              [
              {\eg~\citet{dasgupta2023language}, \citet{wang2023recursively}, Inner Monologue \cite{huang2022inner}}, sys_leaf, text width=27em
              ]
             ]
             [
              Planning Reflection, color=orange!100, fill=orange!40, text=black
              [
              {\eg~Generative Agent \cite{park2023generative}, MORTISE \cite{tang2024enhancing}, \citet{wu2022ai}}, sys_leaf, text width=27em
              ]
             ]
             ]
              [
             Action, color=orange!100, fill=orange!60, text=black[
             {\eg~RoleLLM \cite{wang2023rolellm}, Humanoid Agents \cite{wang2023humanoid}, \citet{shen2024decisionmaking}}, sys_leaf, text width=35.7em
             ]
             ]
             [
             Multi-Modal, color=orange!100, fill=orange!60, text=black[
            {\eg~MPCHAT \cite{ahn2023mpchat}, Narrative Play \cite{zhao2023narrativeplay}, MORTISE \cite{tang2024enhancing}}, sys_leaf, text width=35.7em
             ]
             ]
             

            
            ]

                    
             [Evaluation (\S \ref{sec:mitigating}), color=pink!100, fill=pink!100, text=black
            [
            Perspectives, color=pink!100, fill=pink!60, text=black
            [
            Conversation Ability, color=pink!100, fill=pink!40, text=black[
              {\eg~Linguistic Quality \cite{song-etal-2021-bob,Zheng_Zhang_Huang_Mao_2020}, Coherence \cite{song-etal-2020-generate}}, eval_leaf, text width=27em
              ]
            ]
            [
            Role-Persona \\ Consistency, color=pink!100, fill=pink!40, text=black[
              {\eg~Attributes \cite{zhou2023characterglm,tu2024charactereval}, Relations \cite{chen2023large,shen2024roleeval}}, eval_leaf, text width=27em
              ]
            ]
            [
            Role-Behavior \\ Consistency, color=pink!100, fill=pink!40, text=black[
              {\eg~Conversation Style \cite{tu2024charactereval}, Personality \cite{zhou2023characterglm}}, eval_leaf, text width=27em
              ]
            ]

            [
            Role-Playing \\ Attractiveness, color=pink!100, fill=pink!40, text=black[
              {\eg~Human Likeness \cite{zhou2023characterglm}, Engagement \cite{chen2024compress}, \\Proactivity \cite{zhang2024unveiling}, Empathy \cite{tu2024charactereval}}, eval_leaf, text width=27em
              ]
            ]
            ]
            
            [
            Approaches, color=pink!100, fill=pink!60, text=black
            [
            Automatic Metrics, color=pink!100, fill=pink!40, text=black[
              {\eg~Absolute Metrics \cite{dinan2018wizard}, Multi-choice format \cite{salemi2024lamp}, \\Relative Metrics \cite{song-etal-2021-bob}}, eval_leaf, text width=27em
              ]
            ]
            [
            Human-based, color=pink!100, fill=pink!40, text=black[
              {\eg~Scoring-based \cite{tian2023chatplug}, Ranking-based \cite{chen2023large, chen2024compress}}, eval_leaf, text width=27em
              ]
            ]
            [
            LLM-based, color=pink!100, fill=pink!40, text=black[
              {\eg~\citet{chen2023large}, \citet{yu2024neeko}}, eval_leaf, text width=27em
              ]
            ]

            ]
            ]
           
            ]

        \end{forest}
    }
    \caption{The main content flow and categorization of this survey. 
    \dy{[dy: delete the foundation model]}}
    \label{categorization_of_survey}
\end{figure*}
